Logical Judges Challenge Human Judges on the Strange Case of B.C.-Valjean

On May 12th, 2020, during the course entitled Artificial Intelligence and Jurisdiction Practice organized by the Italian School of Magistracy, more than 70 magistrates followed our demonstration of a Prolog logical judge reasoning on an armed robbery case. Although the implemented logical judge is just an exercise of knowledge representation and simple deductive reasoning, a practical demonstration of an automated reasoning tool to such a large audience of potential end-users represents a first and unique attempt in Italy and, to the best of our knowledge, in the international panorama. In this paper we present the case addressed by the logical judge - a real case already addressed by a human judge in 2015 - and the feedback on the demonstration collected from the attendees.

==> eptcsdata.tex <==
\providecommand{\firstpage}{268}
\providecommand{\publicationstatus}{F. Ricca, A. Russo et al. (Eds.): Proc.\ 36th International Conference \\
on Logic Programming (Technical Communications) 2020 (ICLP 2020)\\
EPTCS 325, 2020, pp.\ \pageref*{FirstPage}--\pageref{LastPage},
doi:\href{http://dx.doi.org/10.4204/EPTCS.325.32}{10.4204/EPTCS.325.32}}
\pdfoutput=1

